BLO-SAM: Bi-level Optimization Based Overfitting-Preventing Finetuning of SAM

The Segment Anything Model (SAM), a foundation model pretrained on millions of images and segmentation masks, has significantly advanced semantic segmentation, a fundamental task in computer vision. Despite its strengths, SAM encounters two major challenges. Firstly, it struggles with segmenting specific objects autonomously, as it relies on users to manually input prompts like points or bounding boxes to identify targeted objects. Secondly, SAM faces challenges in excelling at specific downstream tasks, like medical imaging, due to a disparity between the distribution of its pretraining data, which predominantly consists of general-domain images, and the data used in downstream tasks. Current solutions to these problems, which involve finetuning SAM, often lead to overfitting, a notable issue in scenarios with very limited data, like in medical imaging. To overcome these limitations, we introduce BLO-SAM, which finetunes SAM based on bi-level optimization (BLO). Our approach allows for automatic image segmentation without the need for manual prompts, by optimizing a learnable prompt embedding. Furthermore, it significantly reduces the risk of overfitting by training the model's weight parameters and the prompt embedding on two separate subsets of the training dataset, each at a different level of optimization. We apply BLO-SAM to diverse semantic segmentation tasks in general and medical domains. The results demonstrate BLO-SAM's superior performance over various state-of-the-art image semantic segmentation methods.

==> deprecated.tex <==



\iffalse
\subsection{Foundation models}
Foundation models (FMs), which are first named in~\cite{bommasani2021opportunities}, are regarded as the foundation for various downstream tasks with various data modalities, including natural language processing (NLP)~\cite{chowdhery2022palm,touvron2023llama}, computer vision (CV)~\cite{singh2022flava,yuan2021florence}, biology~\cite{meier2021language,lin2023evolutionary}, etc. FMs are trained on large datasets to capture general knowledge, serving as a reasonable starting point for a variety of applications~\cite{zhou2023comprehensive}. The success of FMs in natural language processing, including applications like ChatGPT~\cite{brown2020language}, encourages further exploration of FMs in computer vision.
For example, an exemplary convolutional neural network (CNN) learns to distinguish various patches from unlabeled data, then transferring these learned representations to common recognition tasks~\cite{dosovitskiy2014discriminative,alexey2016discriminative}.
Later approaches, like MAE~\cite{he2022masked} and SimMIM~\cite{xie2022simmim}, focus on pre-training models using a reconstruction task. They predict patches directly from unmasked data, enabling the models to develop a profound understanding of domain-specific knowledge.
Recently, the Meta AI group introduced a promptable segmentation model~\cite{kirillov2023segment}, the Segment Anything Model (SAM). SAM uses an MAE-pretrained ViT-H~\cite{dosovitskiy2020image} image encoder, a prompt encoder, and a lightweight transformer-based~\cite{liu2021swin} mask decoder to produce high-quality masks for input images. SAM demonstrates significant capabilities across various segmentation tasks without requiring additional training.
Despite their impressive generalization ability, these foundation models struggle to provide accurate predictions in specific areas, like the medical domain~\cite{huang2023visual}, due to the absence of specialized data in the pretraining process.
\fi
